Boundary behavior of analytic functions of two variables via generalized models

We describe a generalization of the notion of a Hilbert space model of a function in the Schur class of the bidisc. This generalization is well adapted to the investigation of boundary behavior at a mild singularity of the function on the 2-torus. We prove the existence of a generalized model with certain properties corresponding to such a singularity and use this result to solve two function-theoretic problems. The first of these is to characterise the directional derivatives of a function in the Schur class at a singular point on the torus for which the Carath\'eodory condition holds. The second is to obtain a representation theorem for functions in the two-variable Pick class analogous to the refined Nevanlinna representation of functions in the one-variable Pick class.

==> notation.tex <==
\section{Notation}\label{notation}

Define $\T$, $\Pi$,  $\Ha$, $\chi=(1,1)\in\T^2$, nontangential approach, $\norm{.}_\infty$, $\dist(\la,\partial\D^2)$.

Define Schur class, Pick class, carapoint of both scalar and operator-valued functions, Julia quotient, inner operator function (unitary on bdry).

Recall that $\lim_{\la\nt\tau} \ph(\la)$ exists for any carapoint $\tau$, has modulus $1$ and is denoted by $\ph(\tau)$.

The {\em Pick class} is the class of analytic functions on $\Pi$ with non-negative imaginary part, that is functions from $\Pi$ to $\Pi^-$.   It will be denoted by $\Pick$.
For $\tau\in\partial (\D^2)$ we define
\beq\label{defHtau}
\Htau = \left\{ \begin{array}{lcl}
    \tau^1\Ha\times \tau^2 \Ha & \mbox{ if } & \tau\in \T^2\\
     \tau^1\mathbb{H}\times \C & & \tau\in\T\times \D \\
    \C\times\tau^2\mathbb{H} & & \tau\in\D\times\T. \end{array} \right.
\eeq
For $\de\in\Htau$ the ray through $\tau$ in direction $-\de$ points into the bidisk and so it makes sense to consider the directional derivative
\[
D_{-\delta}\ph(\tau)= \lim_{t\to 0+} \frac{\ph(\tau-t\delta)-\ph(\tau)}{t}.
\]

